Consistent View Synthesis with Pose-Guided Diffusion Models

Novel view synthesis from a single image has been a cornerstone problem for many Virtual Reality applications that provide immersive experiences. However, most existing techniques can only synthesize novel views within a limited range of camera motion or fail to generate consistent and high-quality novel views under significant camera movement. In this work, we propose a pose-guided diffusion model to generate a consistent long-term video of novel views from a single image. We design an attention layer that uses epipolar lines as constraints to facilitate the association between different viewpoints. Experimental results on synthetic and real-world datasets demonstrate the effectiveness of the proposed diffusion model against state-of-the-art transformer-based and GAN-based approaches.

==> setup/graphicspath.tex <==
\graphicspath{{figures}, {examples}}


==> setup/symbols.tex <==
% Define math symbols that appear in the texts

\def\xi{\mathbf{x}_i}
\def\yi{\mathbf{y}_i}


==> tables/64vs128.tex <==
\begin{table}[t]
    \caption{}
    \label{tab:super_res}
    \centering
    \footnotesize
    \begin{tabular}{l|cccc} 
	    \toprule
		\multirow{2}{*}{Methods} &  \multicolumn{4}{c}{Re10K} \\
		\cmidrule(lr){2-5} & PSNR ($\uparrow$) & SSIM ($\uparrow$) & LPIPS ($\downarrow$) & FID ($\downarrow$) & KID ($\downarrow$) & Style ($\downarrow$)\\
		\midrule
		$64\rightarrow256$ & $22.79$ & $0.69$ & $2.18$ & $56.57$ & $0.019$\\
		$128\rightarrow256$ & $23.59$ & $0.72$ & $1.89$ & $73.78$ & $0.023$\\
		\bottomrule
    \end{tabular}
\end{table}
